Early Fault-Tolerant Quantum Computing

Over the past decade, research in quantum computing has tended to fall into one of two camps: near-term intermediate scale quantum (NISQ) and fault-tolerant quantum computing (FTQC). Yet, a growing body of work has been investigating how to use quantum computers in transition between these two eras. This envisions operating with tens of thousands to millions of physical qubits, able to support fault-tolerant protocols, though operating close to the fault-tolerant threshold. Two challenges emerge from this picture: how to model the performance of devices that are continually improving and how to design algorithms to make the most use of these devices? In this work we develop a model for the performance of early fault-tolerant quantum computing (EFTQC) architectures and use this model to elucidate the regimes in which algorithms suited to such architectures are advantageous. As a concrete example, we show that, for the canonical task of phase estimation, in a regime of moderate scalability and using just over one million physical qubits, the ``reach'' of the quantum computer can be extended (compared to the standard approach) from 90-qubit instances to over 130-qubit instances using a simple early fault-tolerant quantum algorithm, which reduces the number of operations per circuit by a factor of 100 and increases the number of circuit repetitions by a factor of 10,000. This clarifies the role that such algorithms might play in the era of limited-scalability quantum computing.

==> misc.tex <==
\todo[fancyline, color=red]{Athena and PJ explored the question of: can you convey the value of trading circuit repetitions for circuit depth through a fully-costed out utility-scale GSEE instance? We found:}
\begin{itemize}
    \item Over different scalability factors, the physical qubit number is not strongly dependent on $\alpha$ (qubits range over a factor of two or so)
    \item It seemed that by fine-tuning the scalability value and tweaking it around there, the runtime-vs-alpha plot had a minimum runtime at some particular alpha value
    \item For most values of scalability, it seemed that the minimal runtime just corresponded to the largest value of alpha where the error rates were below the required value.
    \item We're deciding to kick the can on this because:
\end{itemize}
